Momentum-based Weight Interpolation of Strong Zero-Shot Models for Continual Learning

Large pre-trained, zero-shot capable models have shown considerable success both for standard transfer and adaptation tasks, with particular robustness towards distribution shifts. In addition, subsequent fine-tuning can considerably improve performance on a selected downstream task. However, through naive fine-tuning, these zero-shot models lose their generalizability and robustness towards distribution shifts. This is a particular problem for tasks such as Continual Learning (CL), where continuous adaptation has to be performed as new task distributions are introduced sequentially. In this work, we showcase that where fine-tuning falls short to adapt such zero-shot capable models, simple momentum-based weight interpolation can provide consistent improvements for CL tasks in both memory-free and memory-based settings. In particular, we find improvements of over $+4\%$ on standard CL benchmarks, while reducing the error to the upper limit of jointly training on all tasks at once in parts by more than half, allowing the continual learner to inch closer to the joint training limits.

==> figures/conv_comp.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{images/conv.png}
    \caption{\textit{Impact on convergence.} Matching performance is reached much earlier, with significantly better overall downstream generalization performance.
    %. Visualization is capped at 100 epochs for qualitative comparability.
    }
    \label{fig:convergence}
\end{figure}

==> figures/firstpage.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{images/figure_1_v2.png}
    \vspace{-6pt}
    \caption{\textit{Language-guidance for better semantic visual alignment.} We leverage language context to better align learned metric spaces with higher-level semantic relations and significantly improve generalization performance.%By leveraging language context, we propose an extension to existing visual similarity learning models that allows for better alignment of learned metric spaces with higher-level semantic relations for significantly improved generalization performance.
    }
    \label{fig:firstpage}
    \vspace{-8pt}
\end{figure}

==> figures/qualitative_retrieval.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/qual_comp.png}
    \vspace{-5pt}
    \caption{\textit{Improved semantic retrieval.} Embedding test classes on CUB200-2011 for models with and without language guidance and evaluating the Top-5 retrieved classes (sorted by semantic similarity) to a query test classes highlights that language-guided models retrieve more samples from semantically related classes.}
    \label{fig:qualitative_retrieval}
    \vspace{-10pt}
\end{figure}

==> figures/setup.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.97\textwidth]{images/setup.png}
    \vspace{-6pt}
    \caption{\textit{Language guidance.} We extend the default DML pipeline for Visual Similarity Learning by embedding either \textbf{(A)} expert class names or \textbf{(B)} top-$k$ ImageNet pseudolabels, which require no additional expert supervision, with a pretrained language model. This provides language similarity matrices $S^\text{lang}$ which are used to guide the structuring of our finegrained visual similarity space generated by $f\circ \phi_\text{ImageNet}$ through distillation-based matching ($\mathcal{L}_\text{match}$ \& $\mathcal{L}_\text{pseudomatch}$) between $S^\text{lang}$ and image similarities $S^\text{img, X}$.
    % \oriol{The figure is really nice. Only if you have a good idea, but the only thing that "bothers" me is (C). A and B are the main methods. C is just a few examples to explain B. Could we group / name things differently so that distinction is clearer without reading caption / text?} \zeynep{I think C could be integrated inside B} \zeynep{how about you remove the car, move the baltimore oriole before the imageNet box (blue box), shift the imagenet blue box and everything to the right of it to the right. the image then is fed to the imagenet, then you can mark the top 3 labels on the blue chart next to the imageNet box, then the rest of the figure in B is the same. remove C.}
    }
    \label{fig:setup}
    \vspace{-5pt}
\end{figure*}

==> figures/tau_task-il-acc.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\scriptsize
\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[
    group style={group size=3 by 1},
    width=5.7cm,
    height=5cm
]
\nextgroupplot[
axis line style={lightgray204},
tick align=outside,
title={Seq-CIFAR-10},
unbounded coords=jump,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{$\tau$},
xmajorticks=true,
xmin=-0.5, xmax=5.5,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4,5},
xticklabels={0.995,0.997,0.999,0.9995,0.9997,0.9999},
xticklabel style={rotate=45,anchor=east},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{Task-IL Accuracy},
ymajorgrids,
ymajorticks=true,
ymin=98.5015, ymax=99.4951666666667,
ytick style={color=darkslategray38}
]
\addplot [line width=1.08pt, steelblue31119180]
table {%
0 99.3766666666667
1 99.37
2 99.4033333333334
3 99.4033333333334
4 99.3966666666667
5 99.39
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
5 nan
5 nan
};
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, only marks]
table{%
x  y
0 99.3766666666667
1 99.37
2 99.4033333333334
3 99.4033333333334
4 99.3966666666667
5 99.39
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
0 99.4266666666667
1 99.4266666666667
2 99.4266666666667
3 99.45
4 99.4433333333333
5 99.3766666666667
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
5 nan
5 nan
};
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, only marks]
table{%
x  y
0 99.4266666666667
1 99.4266666666667
2 99.4266666666667
3 99.45
4 99.4433333333333
5 99.3766666666667
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
0 98.66
1 98.66
2 98.57
3 98.6
4 98.58
5 99.1233333333333
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
5 nan
5 nan
};
\addplot [draw=forestgreen4416044, fill=forestgreen4416044, mark=*, only marks]
table{%
x  y
0 98.66
1 98.66
2 98.57
3 98.6
4 98.58
5 99.1233333333333
};
\addplot [line width=1.08pt, crimson2143940]
table {%
0 98.5533333333333
1 98.5466666666667
2 98.63
3 98.75
4 98.97
5 98.5633333333333
};
\addplot [line width=1.08pt, crimson2143940]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
5 nan
5 nan
};
\addplot [draw=crimson2143940, fill=crimson2143940, mark=*, only marks]
table{%
x  y
0 98.5533333333333
1 98.5466666666667
2 98.63
3 98.75
4 98.97
5 98.5633333333333
};

\nextgroupplot[
axis line style={lightgray204},
tick align=outside,
title={Seq-CIFAR-100},
unbounded coords=jump,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{$\tau$},
xmajorticks=true,
xmin=-0.5, xmax=5.5,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4,5},
xticklabels={0.995,0.997,0.999,0.9995,0.9997,0.9999},
xticklabel style={rotate=45,anchor=east},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{},
ymajorgrids,
ymajorticks=true,
ymin=92.461, ymax=97.719,
ytick style={color=darkslategray38}
]
\addplot [line width=1.08pt, steelblue31119180]
table {%
0 94.9466666666667
1 95.0566666666667
2 96.5266666666667
3 96.77
4 96.9233333333333
5 96.2866666666667
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, steelblue31119180]
table {%
5 nan
5 nan
};
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, only marks]
table{%
x  y
0 94.9466666666667
1 95.0566666666667
2 96.5266666666667
3 96.77
4 96.9233333333333
5 96.2866666666667
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
0 97.3366666666667
1 97.3566666666667
2 97.44
3 97.48
4 97.4133333333333
5 96.6133333333333
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, darkorange25512714]
table {%
5 nan
5 nan
};
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, only marks]
table{%
x  y
0 97.3366666666667
1 97.3566666666667
2 97.44
3 97.48
4 97.4133333333333
5 96.6133333333333
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
0 94.18
1 94.34
2 94.73
3 95.39
4 95.4566666666667
5 95.1433333333333
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, forestgreen4416044]
table {%
5 nan
5 nan
};
\addplot [draw=forestgreen4416044, fill=forestgreen4416044, mark=*, only marks]
table{%
x  y
0 94.18
1 94.34
2 94.73
3 95.39
4 95.4566666666667
5 95.1433333333333
};
\addplot [line width=1.08pt, crimson2143940]
table {%
0 94.2066666666667
1 94.87
2 95.5466666666667
3 95.4066666666667
4 94.89
5 92.7
};
\addplot [line width=1.08pt, crimson2143940]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, crimson2143940]
table {%
5 nan
5 nan
};
\addplot [draw=crimson2143940, fill=crimson2143940, mark=*, only marks]
table{%
x  y
0 94.2066666666667
1 94.87
2 95.5466666666667
3 95.4066666666667
4 94.89
5 92.7
};

\nextgroupplot[
axis line style={lightgray204},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.05,1)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
title={Seq-Tiny-ImageNet},
unbounded coords=jump,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{$\tau$},
xmajorticks=true,
xmin=-0.5, xmax=5.5,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4,5},
xticklabels={0.995,0.997,0.999,0.9995,0.9997,0.9999},
xticklabel style={rotate=45,anchor=east},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{},
ymajorgrids,
ymajorticks=true,
ymin=81.3623333333333, ymax=89.891,
ytick style={color=darkslategray38}
]
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
0 84.83
1 84.8233333333333
2 86.36
3 86.74
4 87.9133333333333
5 88.14
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, steelblue31119180, forget plot]
table {%
5 nan
5 nan
};
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, only marks]
table{%
x  y
0 84.83
1 84.8233333333333
2 86.36
3 86.74
4 87.9133333333333
5 88.14
};
\addlegendentry{DER++ (500)}
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
0 89.1533333333333
1 89.15
2 89.3133333333333
3 89.5033333333333
4 89.45
5 89.0566666666667
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, darkorange25512714, forget plot]
table {%
5 nan
5 nan
};
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, only marks]
table{%
x  y
0 89.1533333333333
1 89.15
2 89.3133333333333
3 89.5033333333333
4 89.45
5 89.0566666666667
};
\addlegendentry{DER++ (5000)}
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
0 81.75
1 81.77
2 83.0666666666667
3 83.54
4 83.65
5 86.4733333333333
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, forestgreen4416044, forget plot]
table {%
5 nan
5 nan
};
\addplot [draw=forestgreen4416044, fill=forestgreen4416044, mark=*, only marks]
table{%
x  y
0 81.75
1 81.77
2 83.0666666666667
3 83.54
4 83.65
5 86.4733333333333
};
\addlegendentry{oEWC}
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
0 83.11
1 83.0933333333333
2 83.06
3 85.1866666666667
4 85.87
5 84.7366666666667
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, crimson2143940, forget plot]
table {%
5 nan
5 nan
};
\addplot [draw=crimson2143940, fill=crimson2143940, mark=*, only marks]
table{%
x  y
0 83.11
1 83.0933333333333
2 83.06
3 85.1866666666667
4 85.87
5 84.7366666666667
};
\addlegendentry{SGD}
\end{groupplot}

\end{tikzpicture}


==> figures/test.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}
\scriptsize
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\pgfplotsset{compat=1.11,
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
       \draw[##1,/tikz/.cd,yshift=-0.25em]
        (0cm,0cm) rectangle (3pt,0.8em);},
   },
}

\begin{axis}[
width=18cm,
height=5cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-1.975, xmax=35.975,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29,30,31,32,33,34},
xticklabel style={rotate=80.0},
xticklabels={
  swin\_base\_patch4\_window7\_224,
  resnetv2\_101x1\_bitm,
  resnetv2\_50x3\_bitm,
  cait\_s24\_224,
  vit\_base\_patch32\_224,
  efficientnet\_b2,
  swsl\_resnext101\_32x4d,
  resnet200d,
  resnetrs200,
  resnet101d,
  regnetz\_d32,
  efficientnet\_b3,
  regnetz\_d8,
  ssl\_resnext101\_32x4d,
  clip,
  ig\_resnext101\_32x16d,
  gcresnext50ts,
  seresnext26d\_32x4d,
  ssl\_resnext101\_32x16d,
  regnety\_064,
  deit\_base\_patch16\_224,
  eca\_resnext26ts,
  efficientnet\_b4,
  resnext26ts,
  regnetx\_064,
  regnetx\_120,
  regnety\_080,
  regnetx\_080,
  resnet34,
  resnetrs420,
  tv\_resnext50\_32x4d,
  gluon\_resnext101\_32x4d,
  regnetz\_c16,
  xception65,
  xception71
},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=0.871120395634379,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.25,0) rectangle (axis cs:0,0.787812288993923);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0}
\addlegendentry{test recall@1}

\draw[draw=none,fill=color0] (axis cs:0.75,0) rectangle (axis cs:1,0.74527346387576);
\draw[draw=none,fill=color0] (axis cs:1.75,0) rectangle (axis cs:2,0.715732613099257);
\draw[draw=none,fill=color0] (axis cs:2.75,0) rectangle (axis cs:3,0.62221471978393);
\draw[draw=none,fill=color0] (axis cs:3.75,0) rectangle (axis cs:4,0.613099257258609);
\draw[draw=none,fill=color0] (axis cs:4.75,0) rectangle (axis cs:5,0.581532748143146);
\draw[draw=none,fill=color0] (axis cs:5.75,0) rectangle (axis cs:6,0.576130992572586);
\draw[draw=none,fill=color0] (axis cs:6.75,0) rectangle (axis cs:7,0.574611748818366);
\draw[draw=none,fill=color0] (axis cs:7.75,0) rectangle (axis cs:8,0.558237677245105);
\draw[draw=none,fill=color0] (axis cs:8.75,0) rectangle (axis cs:9,0.557224848075625);
\draw[draw=none,fill=color0] (axis cs:9.75,0) rectangle (axis cs:10,0.550303848750844);
\draw[draw=none,fill=color0] (axis cs:10.75,0) rectangle (axis cs:11,0.545070898041864);
\draw[draw=none,fill=color0] (axis cs:11.75,0) rectangle (axis cs:12,0.526839972991222);
\draw[draw=none,fill=color0] (axis cs:12.75,0) rectangle (axis cs:13,0.522451046590142);
\draw[draw=none,fill=color0] (axis cs:13.75,0) rectangle (axis cs:14,0.518230925050641);
\draw[draw=none,fill=color0] (axis cs:14.75,0) rectangle (axis cs:15,0.511647535449021);
\draw[draw=none,fill=color0] (axis cs:15.75,0) rectangle (axis cs:16,0.511309925725861);
\draw[draw=none,fill=color0] (axis cs:16.75,0) rectangle (axis cs:17,0.49645509790682);
\draw[draw=none,fill=color0] (axis cs:17.75,0) rectangle (axis cs:18,0.492572586090479);
\draw[draw=none,fill=color0] (axis cs:18.75,0) rectangle (axis cs:19,0.491222147197839);
\draw[draw=none,fill=color0] (axis cs:19.75,0) rectangle (axis cs:20,0.487339635381499);
\draw[draw=none,fill=color0] (axis cs:20.75,0) rectangle (axis cs:21,0.481769074949359);
\draw[draw=none,fill=color0] (axis cs:21.75,0) rectangle (axis cs:22,0.480081026333558);
\draw[draw=none,fill=color0] (axis cs:22.75,0) rectangle (axis cs:23,0.468939905469277);
\draw[draw=none,fill=color0] (axis cs:23.75,0) rectangle (axis cs:24,0.458474004051317);
\draw[draw=none,fill=color0] (axis cs:24.75,0) rectangle (axis cs:25,0.454760297096556);
\draw[draw=none,fill=color0] (axis cs:25.75,0) rectangle (axis cs:26,0.454422687373396);
\draw[draw=none,fill=color0] (axis cs:26.75,0) rectangle (axis cs:27,0.447839297771776);
\draw[draw=none,fill=color0] (axis cs:27.75,0) rectangle (axis cs:28,0.446320054017556);
\draw[draw=none,fill=color0] (axis cs:28.75,0) rectangle (axis cs:29,0.432984469952735);
\draw[draw=none,fill=color0] (axis cs:29.75,0) rectangle (axis cs:30,0.427751519243754);
\draw[draw=none,fill=color0] (axis cs:30.75,0) rectangle (axis cs:31,0.402430790006752);
\draw[draw=none,fill=color0] (axis cs:31.75,0) rectangle (axis cs:32,0.299291019581364);
\draw[draw=none,fill=color0] (axis cs:32.75,0) rectangle (axis cs:33,0.141964888588791);
\draw[draw=none,fill=color0] (axis cs:33.75,0) rectangle (axis cs:34,0.0577312626603646);
\draw[draw=none,fill=color1] (axis cs:0,0) rectangle (axis cs:0.25,0.829638472032742);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1}
\addlegendentry{train recall@1}

\draw[draw=none,fill=color1] (axis cs:1,0) rectangle (axis cs:1.25,0.79399727148704);
\draw[draw=none,fill=color1] (axis cs:2,0) rectangle (axis cs:2.25,0.783424283765348);
\draw[draw=none,fill=color1] (axis cs:3,0) rectangle (axis cs:3.25,0.733117326057299);
\draw[draw=none,fill=color1] (axis cs:4,0) rectangle (axis cs:4.25,0.700886766712142);
\draw[draw=none,fill=color1] (axis cs:5,0) rectangle (axis cs:5.25,0.723567530695771);
\draw[draw=none,fill=color1] (axis cs:6,0) rectangle (axis cs:6.25,0.72612551159618);
\draw[draw=none,fill=color1] (axis cs:7,0) rectangle (axis cs:7.25,0.714017735334243);
\draw[draw=none,fill=color1] (axis cs:8,0) rectangle (axis cs:8.25,0.707878581173261);
\draw[draw=none,fill=color1] (axis cs:9,0) rectangle (axis cs:9.25,0.702933151432469);
\draw[draw=none,fill=color1] (axis cs:10,0) rectangle (axis cs:10.25,0.699010914051842);
\draw[draw=none,fill=color1] (axis cs:11,0) rectangle (axis cs:11.25,0.693553888130969);
\draw[draw=none,fill=color1] (axis cs:12,0) rectangle (axis cs:12.25,0.665586630286494);
\draw[draw=none,fill=color1] (axis cs:13,0) rectangle (axis cs:13.25,0.672237380627558);
\draw[draw=none,fill=color1] (axis cs:14,0) rectangle (axis cs:14.25,0.6268758526603);
\draw[draw=none,fill=color1] (axis cs:15,0) rectangle (axis cs:15.25,0.64887448840382);
\draw[draw=none,fill=color1] (axis cs:16,0) rectangle (axis cs:16.25,0.658594815825375);
\draw[draw=none,fill=color1] (axis cs:17,0) rectangle (axis cs:17.25,0.64887448840382);
\draw[draw=none,fill=color1] (axis cs:18,0) rectangle (axis cs:18.25,0.654331514324693);
\draw[draw=none,fill=color1] (axis cs:19,0) rectangle (axis cs:19.25,0.653990450204638);
\draw[draw=none,fill=color1] (axis cs:20,0) rectangle (axis cs:20.25,0.649897680763984);
\draw[draw=none,fill=color1] (axis cs:21,0) rectangle (axis cs:21.25,0.631650750341064);
\draw[draw=none,fill=color1] (axis cs:22,0) rectangle (axis cs:22.25,0.655695770804911);
\draw[draw=none,fill=color1] (axis cs:23,0) rectangle (axis cs:23.25,0.598226466575716);
\draw[draw=none,fill=color1] (axis cs:24,0) rectangle (axis cs:24.25,0.61681446111869);
\draw[draw=none,fill=color1] (axis cs:25,0) rectangle (axis cs:25.25,0.611527967257845);
\draw[draw=none,fill=color1] (axis cs:26,0) rectangle (axis cs:26.25,0.620225102319236);
\draw[draw=none,fill=color1] (axis cs:27,0) rectangle (axis cs:27.25,0.621418826739427);
\draw[draw=none,fill=color1] (axis cs:28,0) rectangle (axis cs:28.25,0.617496589358799);
\draw[draw=none,fill=color1] (axis cs:29,0) rectangle (axis cs:29.25,0.620395634379263);
\draw[draw=none,fill=color1] (axis cs:30,0) rectangle (axis cs:30.25,0.609652114597544);
\draw[draw=none,fill=color1] (axis cs:31,0) rectangle (axis cs:31.25,0.57912687585266);
\draw[draw=none,fill=color1] (axis cs:32,0) rectangle (axis cs:32.25,0.370736698499318);
\draw[draw=none,fill=color1] (axis cs:33,0) rectangle (axis cs:33.25,0.189972714870396);
\draw[draw=none,fill=color1] (axis cs:34,0) rectangle (axis cs:34.25,0.0678717598908595);
\end{axis}

\end{tikzpicture}


==> figures/umap.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{example-image-a}
    \caption{\textit{Qualitative UMAP or nearest neighbour retrieval examples.} Reviewers usually ask for a very useless umap of different embedding spaces. Can be included here.}
    \label{fig:umap}
\end{figure}

==> tables/ablation_on_distillation_methods.tex <==
\begin{table}[t]
    \caption{\textit{Including language context.} Distillation of relative language embedding alignments offers the most benefits.}
\vspace{-5pt}
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \resizebox{0.43\textwidth}{!}{
  \begin{tabular}{l || c | c || c | c }
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
     \midrule
     \multirow{2}{*}{\textsc{Methods} $\downarrow$} & \multirow{2}{*}{R@1} & mAP & \multirow{2}{*}{R@1} & mAP \\
     & & @1000 & & @1000 \\
    \midrule
    \rowcolor{vlightgray}    
    Baseline & 62.8 $\pm$ 0.2 & 31.1 $\pm$ 0.2 & 81.6 $\pm$ 0.3 & 31.7 $\pm$ 0.1 \\
    \rowcolor{vvlightgray}    
    + \textit{ELG} & \textbf{67.3 $\pm$ 0.2} & \textbf{34.8 $\pm$ 0.2} & \textbf{85.3 $\pm$ 0.1} & \textbf{32.7 $\pm$ 0.2} \\
    \midrule    
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(a) Vision-Language representation matching}} \\         
    \hline
    DeVise-Style & 64.2 $\pm$ 0.3 & 32.0 $\pm$ 0.1 & 83.9 $\pm$ 0.3 & 32.2 $\pm$ 0.2 \\    
    ViT Prediction & 65.1 $\pm$ 0.4 & 33.0 $\pm$ 0.1 & 83.2 $\pm$ 0.2 & 32.0 $\pm$ 0.3 \\
    CLIP-style & 63.7 $\pm$ 0.4 & 31.9 $\pm$ 0.6 & 83.2 $\pm$ 0.4 & 32.2 $\pm$ 0.3 \\
    \hline
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(b) Methods of incorporation}} \\    
    \hline    
    Row-wise L2 & 65.2 $\pm$ 0.2 & 32.4 $\pm$ 0.2 & 84.4 $\pm$ 0.3 & 32.1 $\pm$ 0.1 \\
    Full Similarity & 64.9 $\pm$ 0.3 & 32.3 $\pm$ 0.2 & 84.0 $\pm$ 0.1 & 32.0 $\pm$ 0.3 \\    
    % Eucl. \& Cosine & 67.1 $\pm$ 0.2 & 33.3 $\pm$ 0.2 & \textbf{85.5 $\pm$ 0.4} & \textbf{33.6 $\pm$ 0.3} \\    
    Mining mask & 64.1 $\pm$ 0.3 & 32.6 $\pm$ 0.2 & 81.9 $\pm$ 0.2 & 32.3 $\pm$ 0.4 \\    
    Weight scaling & 59.2 $\pm$ 0.5 & 29.9 $\pm$ 0.4 & 74.6 $\pm$ 0.5 & 26.0 $\pm$ 0.8 \\    
    No stop grad. & 66.3 $\pm$ 0.4 & 34.1 $\pm$ 0.2 & 83.6 $\pm$ 0.2 & 30.8 $\pm$ 0.2 \\      
    \bottomrule
    \end{tabular}}
    \label{tab:architecture_ablations}
    \vspace{-6pt}
 \end{table}


==> tables/all_lang_models.tex <==
\begin{table}[h!]
    \caption{\textit{Models vs. guidance quality.} Performance improves regardless of the exact large pretrained language model. Strong improvements can even be achieved through large-scale pretrained word embeddings such as FastText \cite{fasttext} and GloVe \cite{glove}. However, using less transferable word hierarchies falls short in comparison.}
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \begin{tabular}{l || c | c || c | c }
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
     \midrule
     \multirow{2}{*}{\textsc{Models} $\downarrow$} & \multirow{2}{*}{R@1} & mAP & \multirow{2}{*}{R@1} & mAP\\
      &  & @1000 & & @1000\\
    \midrule
    \rowcolor{vlightgray}
    \textbf{Baseline} & 62.8 $\pm$ 0.2 & 31.1 $\pm$ 0.3 & 81.6 $\pm$ 0.3 & 31.7 $\pm$ 0.1\\ 
    \rowcolor{vvlightgray}    
    + CLIP-L \cite{clip} & 67.3 $\pm$ 0.2 & \textbf{34.8 $\pm$ 0.2} & 85.3 $\pm$ 0.1 & \textbf{32.7 $\pm$ 0.2} \\
    % \hline
    % + $\mathbb{S}^{N-1}\left(\mathcal{N}(0,1)\right)$ & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
    \midrule        
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(a) Language Models}} \\
    \hline
    + BERT \cite{bert} & 66.9 $\pm$ 0.3 & 33.5 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.1\\
    + DistBert \cite{distilbert} & 66.7 $\pm$ 0.1 & 33.4 $\pm$ 0.2 & 85.4 $\pm$ 0.4 & 32.4 $\pm$ 0.1\\    
    + Roberta-B \cite{roberta} & 67.0 $\pm$ 0.2 & 33.8 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.3\\
    + Roberta-L \cite{roberta} & 67.3 $\pm$ 0.2 & 33.9 $\pm$ 0.3 & 85.1 $\pm$ 0.2 & 32.4 $\pm$ 0.2\\
    + DistRoberta \cite{huggingface} & 66.0 $\pm$ 0.2 & 32.2 $\pm$ 0.2 & 85.0 $\pm$ 0.3 & 32.1 $\pm$ 0.2\\
    + Reformer \cite{Kitaev2020Reformer} & 66.7 $\pm$ 0.1 & 33.1 $\pm$ 0.1 & 85.5 $\pm$ 0.2 & 32.0 $\pm$ 0.2\\
    + MPNet \cite{mpnet} & 66.2 $\pm$ 0.3 & 32.3 $\pm$ 0.2 & 85.4 $\pm$ 0.2 & 32.3 $\pm$ 0.3\\
    + GPT2 \cite{gpt2} & 67.0 $\pm$ 0.3 & 33.7 $\pm$ 0.1 & 84.8 $\pm$ 0.4 & 32.4 $\pm$ 0.1\\
    \hline
    + Top 3 & \textbf{67.5 $\pm$ 0.2} & 34.5 $\pm$ 0.3 & \textbf{85.6 $\pm$ 0.3} & 32.5 $\pm$ 0.3\\   
    \bottomrule
    \end{tabular}
    \label{supp:tab:choice_of_language_models}
 \end{table}

==> tables/choice_of_language_models.tex <==
\begin{table}[t]
    \caption{\textit{Model guidance quality.} Performance improves regardless of the exact language model and even with large-scale pretrained word embeddings s.a. FastText \cite{fasttext} and GloVe \cite{glove}. However, less transferable word hierarchies fall short in comparison.}
\vspace{-5pt}    
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \resizebox{0.43\textwidth}{!}{
  \begin{tabular}{l || c | c || c | c }
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
     \midrule
     \multirow{2}{*}{\textsc{Models} $\downarrow$} & \multirow{2}{*}{R@1} & mAP & \multirow{2}{*}{R@1} & mAP\\
      &  & @1000 & & @1000\\
    \midrule
    \rowcolor{vlightgray}
    \textbf{Baseline} & 62.8 $\pm$ 0.2 & 31.1 $\pm$ 0.3 & 81.6 $\pm$ 0.3 & 31.7 $\pm$ 0.1\\ 
    \rowcolor{vvlightgray}    
    + CLIP-L \cite{clip} & 67.3 $\pm$ 0.2 & \textbf{34.8 $\pm$ 0.2} & 85.3 $\pm$ 0.1 & \textbf{32.7 $\pm$ 0.2} \\
    % \hline
    % + $\mathbb{S}^{N-1}\left(\mathcal{N}(0,1)\right)$ & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
    \midrule        
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(a) Language Models}} \\
    \hline
    + BERT \cite{bert} & 66.9 $\pm$ 0.3 & 33.5 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.1\\
    % + DistBert \cite{distilbert} & 66.7 $\pm$ 0.1 & 33.4 $\pm$ 0.2 & 85.4 $\pm$ 0.4 & 32.4 $\pm$ 0.1\\    
    % + Roberta-B \cite{roberta} & 67.0 $\pm$ 0.2 & 33.8 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.3\\
    + Roberta-L \cite{roberta} & 67.3 $\pm$ 0.2 & 33.9 $\pm$ 0.3 & 85.1 $\pm$ 0.2 & 32.4 $\pm$ 0.2\\
    % + DistRoberta \cite{huggingface} & 66.0 $\pm$ 0.2 & 32.2 $\pm$ 0.2 & 85.0 $\pm$ 0.3 & 32.1 $\pm$ 0.2\\
    + Reformer \cite{Kitaev2020Reformer} & 66.7 $\pm$ 0.1 & 33.1 $\pm$ 0.1 & 85.5 $\pm$ 0.2 & 32.0 $\pm$ 0.2\\
    % + MPNet \cite{mpnet} & 66.2 $\pm$ 0.3 & 32.3 $\pm$ 0.2 & 85.4 $\pm$ 0.2 & 32.3 $\pm$ 0.3\\
    + GPT2 \cite{gpt2} & 67.0 $\pm$ 0.3 & 33.7 $\pm$ 0.1 & 84.8 $\pm$ 0.4 & 32.4 $\pm$ 0.1\\
    \hline
    + Top 3 & \textbf{67.5 $\pm$ 0.2} & 34.5 $\pm$ 0.3 & \textbf{85.6 $\pm$ 0.3} & 32.5 $\pm$ 0.3\\   
    \hline
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(b) Word Embeddings}} \\
    \hline
    + FastText \cite{fasttext} & 66.9 $\pm$ 0.3 & 33.7 $\pm$ 0.3 & 85.2 $\pm$ 0.1 & \textbf{32.7 $\pm$ 0.1}\\
    + GloVe \cite{glove} & 66.1 $\pm$ 0.2 & 33.1 $\pm$ 0.3 & 85.0 $\pm$ 0.2 & 32.1 $\pm$ 0.3\\    
    \hline
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(c) Word Hierarchies}} \\
    + WordNet \cite{wordnet} & 63.7 $\pm$ 0.2 & 31.3 $\pm$ 0.2 & 82.5 $\pm$ 0.3 & 31.0 $\pm$ 0.2\\
    + HierMatch \cite{hiermatch} & 64.8 $\pm$ 0.3 & 32.2 $\pm$ 0.1 & 82.8 $\pm$ 0.2 & 31.8 $\pm$ 0.1\\
    \bottomrule
    \end{tabular}}
    \label{tab:choice_of_language_models}
    \vspace{-8pt}
 \end{table}
 
 
 
 
 \begin{table}[t]
    \caption{\textit{Model guidance quality.} Performance improves regardless of the exact language model and even with large-scale pretrained word embeddings s.a. FastText \cite{fasttext} and GloVe \cite{glove}. However, less transferable word hierarchies fall short in comparison.}
\vspace{-5pt}    
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \resizebox{0.43\textwidth}{!}{
  \begin{tabular}{l || c | c || c | c }
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
     \midrule
     \textsc{Models} $\downarrow$ & R@1 & mAP & R@1 & mAP\\
    \midrule        
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(a) Language Models}} \\
    \hline
    + CLIP-L \cite{clip} & 67.3 $\pm$ 0.2 & \textbf{34.8 $\pm$ 0.2} & 85.3 $\pm$ 0.1 & \textbf{32.7 $\pm$ 0.2} \\
    + BERT \cite{bert} & 66.9 $\pm$ 0.3 & 33.5 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.1\\
    % + DistBert \cite{distilbert} & 66.7 $\pm$ 0.1 & 33.4 $\pm$ 0.2 & 85.4 $\pm$ 0.4 & 32.4 $\pm$ 0.1\\    
    % + Roberta-B \cite{roberta} & 67.0 $\pm$ 0.2 & 33.8 $\pm$ 0.2 & 84.9 $\pm$ 0.1 & 32.3 $\pm$ 0.3\\
    + Reformer \cite{Kitaev2020Reformer} & 66.7 $\pm$ 0.1 & 33.1 $\pm$ 0.1 & 85.5 $\pm$ 0.2 & 32.0 $\pm$ 0.2\\
    % + MPNet \cite{mpnet} & 66.2 $\pm$ 0.3 & 32.3 $\pm$ 0.2 & 85.4 $\pm$ 0.2 & 32.3 $\pm$ 0.3\\
    \hline
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(b) Word Embeddings}} \\
    \hline
    + FastText \cite{fasttext} & 66.9 $\pm$ 0.3 & 33.7 $\pm$ 0.3 & 85.2 $\pm$ 0.1 & \textbf{32.7 $\pm$ 0.1}\\
    + GloVe \cite{glove} & 66.1 $\pm$ 0.2 & 33.1 $\pm$ 0.3 & 85.0 $\pm$ 0.2 & 32.1 $\pm$ 0.3\\    
    \hline
    \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{(c) Word Hierarchies}} \\
    + WordNet \cite{wordnet} & 63.7 $\pm$ 0.2 & 31.3 $\pm$ 0.2 & 82.5 $\pm$ 0.3 & 31.0 $\pm$ 0.2\\
    + HierMatch \cite{hiermatch} & 64.8 $\pm$ 0.3 & 32.2 $\pm$ 0.1 & 82.8 $\pm$ 0.2 & 31.8 $\pm$ 0.1\\
    \bottomrule
    \end{tabular}}
    \label{tab:choice_of_language_models}
    \vspace{-8pt}
 \end{table}

==> tables/dense_captions.tex <==
\begin{table}[t]
\caption{\textit{Do dense captions help?} We find class knowledge to be more valuable than generic image captions for generalization.}
\vspace{-5pt}
\footnotesize
\setlength\tabcolsep{1.4pt}
\centering
%\begin{tabular}{l|c|ccc|c}
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{l || c | c || c | c }
\toprule
\multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
\midrule
\multirow{2}{*}{\textsc{Approaches} $\downarrow$} & \multirow{2}{*}{R@1} & mAP & \multirow{2}{*}{R@1} & mAP\\
&  & @1000 & & @1000\\
\midrule
\rowcolor{vlightgray}
Baseline & 62.8 $\pm$ 0.2 & 31.1 $\pm$ 0.2 & 81.6 $\pm$ 0.3 & 31.7 $\pm$ 0.1 \\
\rowcolor{vvlightgray}    
+ \textit{ELG} & 67.3 $\pm$ 0.2 & 34.8 $\pm$ 0.2 & 85.3 $\pm$ 0.1 & 32.7 $\pm$ 0.2 \\
\midrule
Caption & 64.9 $\pm$ 0.4 & 32.2 $\pm$ 0.2 & 84.9 $\pm$ 0.2 & 31.9 $\pm$ 0.3 \\
Caption + insertion & 67.1 $\pm$ 0.2 & 34.3 $\pm$ 0.1 & 85.4 $\pm$ 0.2 & 32.7 $\pm$ 0.3 \\
Classname only & 67.3 $\pm$ 0.3 & 34.7 $\pm$ 0.1 & 85.1 $\pm$ 0.2 & 32.5 $\pm$ 0.1 \\
Other primers & 67.4 $\pm$ 0.1 & 34.7 $\pm$ 0.2 & 85.5 $\pm$ 0.3 & 32.7 $\pm$ 0.1 \\
\bottomrule
\end{tabular}}
\label{tab:caption_ablations}
\vspace{-8pt}
\end{table}


==> tables/plangg.tex <==
\begin{table}[h!]
\caption{\textit{Ablations on Pseudolabel guidance.} More pseudolabels per class improve generalization performance, with class-level pseudolabelling and distillation from a single average language similarity matrix offering highest improvements.}
\footnotesize
\setlength\tabcolsep{1.4pt}
\centering
%\begin{tabular}{l|c|ccc|c}
\begin{tabular}{l || c | c || c | c }
\toprule
\multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} \\
\midrule
\multirow{2}{*}{\textsc{Approaches} $\downarrow$} & \multirow{2}{*}{R@1} & mAP & \multirow{2}{*}{R@1} & mAP\\
&  & @1000 & & @1000\\
\midrule
\rowcolor{vlightgray}
Baseline & 62.8 $\pm$ 0.2 & 31.1 $\pm$ 0.2 & 81.6 $\pm$ 0.3 & 31.7 $\pm$ 0.1 \\
\rowcolor{vvlightgray}    
+ \textit{ELG} & 67.3 $\pm$ 0.2 & 34.8 $\pm$ 0.2 & 85.3 $\pm$ 0.1 & 32.7 $\pm$ 0.2 \\
\midrule
\multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{Number of pseudolabels}} \\
\hline
+ \textit{PLG} & 66.2 $\pm$ 0.6 & 33.8 $\pm$ 0.2 & 85.2 $\pm$ 0.1 & 32.7 $\pm$ 0.1 \\    
% + \textit{plangg} (Top-2) & 66.6 $\pm$ 0.3 & 34.1 $\pm$ 0.2 & 85.2 $\pm$ 0.2 & 32.6 $\pm$ 0.1 \\   
+ \textit{PLG} (Top-5) & 67.1 $\pm$ 0.4 & 34.6 $\pm$ 0.5 & 85.4 $\pm$ 0.2 & 32.8 $\pm$ 0.2 \\   
+ \textit{PLG} (Top-10) & 67.2 $\pm$ 0.2 & 34.5 $\pm$ 0.3 & 85.3 $\pm$ 0.2 & 32.4 $\pm$ 0.3 \\   
+ \textit{PLG} (Top-20) & 67.0 $\pm$ 0.1 & 34.5 $\pm$ 0.2 & 84.9 $\pm$ 0.4 & 32.1 $\pm$ 0.3 \\   
\midrule
\multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{Word Hierarchies}} \\
\textit{PLG}+WordNet (Top-5) & 64.4 $\pm$ 0.1 & 31.5 $\pm$ 0.2 & 82.9 $\pm$ 0.2 & 31.3 $\pm$ 0.2\\
\textit{pseudo}-HierMatch & 65.0 $\pm$ 0.2 & 32.3 $\pm$ 0.2 & 82.8 $\pm$ 0.3 & 31.6 $\pm$ 0.2\\
\hline
\multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{Different pseudolabel matching methods}} \\
\hline
Sample (Top-5) & 67.0 $\pm$ 0.1 & 34.2 $\pm$ 0.1 & 85.2 $\pm$ 0.2 & 32.2 $\pm$ 0.3 \\   
Dense (Top-5) & 67.0 $\pm$ 0.2 & 33.7 $\pm$ 0.4 & 84.0 $\pm$ 0.1 & 31.5 $\pm$ 0.4 \\   
Multi (Top-5) & 67.2 $\pm$ 0.1 & 34.3 $\pm$ 0.2 & 85.1 $\pm$ 0.2 & 32.2 $\pm$ 0.1 \\   
Dense + Multi & 66.0 $\pm$ 0.3 & 34.1 $\pm$ 0.2 & 84.3 $\pm$ 0.3 & 31.9 $\pm$ 0.2 \\   
\bottomrule
\end{tabular}
\label{tab:plangg_ablations}
\end{table}


==> tables/relative_improvements.tex <==
\begin{table*}[t]
    \caption{\textit{Relative comparison.} We follow protocols proposed in \cite{roth2020revisiting}\protect\footnotemark, with no learning rate scheduling, to ensure exact comparability. The results show significant improvements on CUB200 and CARS196 when language-guidance is applied (with expert- and pseudolabels). ($^*$) For SOP, only 12 superlabels are given for 11,318 training classes. Similarly, SOP only contains very few samples per class, making pseudolabel class estimates very noisy. This makes the benefits of language guidance limited.}
\vspace{-5pt}    
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \resizebox{0.95\textwidth}{!}{
  \begin{tabular}{l || c | c | c || c | c| c || c | c | c}
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{3}{c}{\textsc{CUB200-2011}} & \multicolumn{3}{c}{\textsc{CARS196}} & \multicolumn{3}{c}{\textsc{SOP}($^*$)} \\
     \midrule
     \textsc{Approaches} $\downarrow$ & R@1 & NMI & mAP@1000 & R@1 & NMI & mAP@1000 & R@1 & NMI & mAP@1000\\
    \midrule
    \rowcolor{vvlightgray} 
    \textbf{Multisimilarity} & 62.8 $\pm$ 0.2 & 67.8 $\pm$ 0.4 & 31.1 $\pm$ 0.3 & 81.6 $\pm$ 0.3 & 69.6 $\pm$ 0.5 & 31.7 $\pm$ 0.1 & 76.0 $\pm$ 0.1  & 89.4 $\pm$ 0.1  & 43.3 $\pm$ 0.1 \\
    \hline
    +\textit{ELG} & 67.3 $\pm$ 0.2 & 69.6 $\pm$ 0.6 & 34.8 $\pm$ 0.2 & 85.3 $\pm$ 0.1 & 71.7 $\pm$ 0.2 & 32.7 $\pm$ 0.2 & 76.0 $\pm$ 0.2  & 89.5 $\pm$ 0.1  & 43.5 $\pm$ 0.1 \\ 
    % +\textit{PLG} Top-1 & 66.2 $\pm$ 0.6 & 68.4 $\pm$ 0.3 & 33.8 $\pm$ 0.2 & 85.2 $\pm$ 0.1 & 71.1 $\pm$ 0.3 & 32.7 $\pm$ 0.1 & 76.1 $\pm$ 0.2  & 89.4 $\pm$ 0.2  & 43.4 $\pm$ 0.1 \\ 
    +\textit{PLG} Top-5 & 67.1 $\pm$ 0.4 & 69.6 $\pm$ 0.6 & 34.6 $\pm$ 0.5 & 85.4 $\pm$ 0.2 & 71.3 $\pm$ 0.1 & 32.8 $\pm$ 0.2 & 76.4 $\pm$ 0.1  & 89.6 $\pm$ 0.1  & 43.7 $\pm$ 0.1 \\ 
    % +\textit{PLG} Top-5 No Mask &&&&&&&&&\\
    \midrule 
    \rowcolor{vvlightgray} 
    \textbf{Margin}, $\beta=1.2$ & 62.7 $\pm$ 0.6 & 68.0 $\pm$ 0.3 & 32.2 $\pm$ 0.3 & 79.4 $\pm$ 0.5 & 66.6 $\pm$ 0.7 & 32.8 $\pm$ 0.2 & 78.0 $\pm$ 0.3  & 90.3 $\pm$ 0.2  & 46.3 $\pm$ 0.2 \\ 
    \hline
    +\textit{ELG} & 65.3 $\pm$ 0.5 & 68.5 $\pm$ 0.4 & 33.5 $\pm$ 0.3 & 83.2 $\pm$ 0.5 & 69.0 $\pm$ 0.6 & 33.4 $\pm$ 0.3 & 77.8 $\pm$ 0.1  & 90.2 $\pm$ 0.1  & 46.1 $\pm$ 0.1 \\ 
    % +\textit{PLG} Top-1 & 64.9 $\pm$ 0.4 & 68.4 $\pm$ 0.4 & 33.0 $\pm$ 0.3 & 83.2 $\pm$ 0.4 & 68.7 $\pm$ 0.7 & 33.5 $\pm$ 0.3 & 78.1 $\pm$ 0.2  & 90.2 $\pm$ 0.3  & 46.3 $\pm$ 0.1 \\ 
    +\textit{PLG} Top-5 & 65.2 $\pm$ 0.5 & 68.5 $\pm$ 0.4 & 33.5 $\pm$ 0.3 & 83.4 $\pm$ 0.4 & 69.1 $\pm$ 0.4 & 33.7 $\pm$ 0.3 & 78.3 $\pm$ 0.2  & 90.3 $\pm$ 0.2  & 46.5 $\pm$ 0.1 \\ 
    \midrule 
    \rowcolor{vvlightgray} 
    \textbf{Multisimilarity + S2SD} & 67.7 $\pm$ 0.3 & 71.5 $\pm$ 0.2 & 35.5 $\pm$ 0.2 & 86.5 $\pm$ 0.1 & 71.4 $\pm$ 0.4 & 35.1 $\pm$ 0.3 & 77.7 $\pm$ 0.2  & 89.9 $\pm$ 0.1  & 45.3 $\pm$ 0.3 \\ 
    \hline
    +\textit{ELG} & 68.9 $\pm$ 0.4 & 72.5 $\pm$ 0.3 & 36.4 $\pm$ 0.5 & 88.2 $\pm$ 0.2 & 72.0 $\pm$ 0.1 & 36.0 $\pm$ 0.1 & 77.8 $\pm$ 0.1  & 90.0 $\pm$ 0.2  & 45.3 $\pm$ 0.2 \\ 
    % +\textit{PLG} Top-1 & 68.7 $\pm$ 0.4 & 72.4 $\pm$ 0.4 & 36.2 $\pm$ 0.5 & 88.4 $\pm$ 0.2 & 72.4 $\pm$ 0.3 & 36.2 $\pm$ 0.2 & 77.9 $\pm$ 0.2  & 90.0 $\pm$ 0.2  & 45.4 $\pm$ 0.2 \\ 
    +\textit{PLG} Top-5 & 69.0 $\pm$ 0.4 & 72.4 $\pm$ 0.2 & 36.6 $\pm$ 0.3 & 88.4 $\pm$ 0.3 & 72.4 $\pm$ 0.2 & 36.2 $\pm$ 0.2 & 78.0 $\pm$ 0.1  & 90.0 $\pm$ 0.1  & 45.6 $\pm$ 0.1 \\ 
    \bottomrule 

    \end{tabular}}
    \label{tab:supp_relative_results}
 \end{table*}




==> tables/relative_improvements_small.tex <==
\begin{table}[t]
    \caption{\textit{Relative comparison.} We follow protocols proposed in \cite{roth2020revisiting}\protect\footnotemark, with no learning rate scheduling, to ensure exact comparability. The results show significant improvements when language-guidance is applied. ($^*$) For SOP, only 12 superlabels are given for 11,318 training classes, with very few samples per class. This limits the benefits of language guidance.}
\vspace{-5pt}    
 \footnotesize
  \setlength\tabcolsep{1.4pt}
  \centering
  %\begin{tabular}{l|c|ccc|c}
  \resizebox{0.43\textwidth}{!}{
  \begin{tabular}{l || c | c | c}
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks}$\rightarrow$} & \multicolumn{1}{c}{\textsc{CUB200}} & \multicolumn{1}{c}{\textsc{CARS196}} & \multicolumn{1}{c}{\textsc{SOP}($^*$)} \\
     \midrule
     \textsc{Approaches} $\downarrow$ & R@1 & R@1 & R@1 \\
    \midrule
    \rowcolor{vvlightgray} 
    \textbf{Multisimilarity} & 62.8 $\pm$ 0.2 & 81.6 $\pm$ 0.3 & 76.0 $\pm$ 0.1\\
    \hline
    +\textit{ELG} & 67.3 $\pm$ 0.2& 85.3 $\pm$ 0.1 & 76.0 $\pm$ 0.2\\ 
    % +\textit{pELG} Top-1 & 66.2 $\pm$ 0.6 & 68.4 $\pm$ 0.3 & 33.8 $\pm$ 0.2 & 85.2 $\pm$ 0.1 & 71.1 $\pm$ 0.3 & 32.7 $\pm$ 0.1 & 76.1 $\pm$ 0.2  & 89.4 $\pm$ 0.2  & 43.4 $\pm$ 0.1 \\ 
    +\textit{PLG} Top-5 & 67.1 $\pm$ 0.4 & 85.4 $\pm$ 0.2 & 76.4 $\pm$ 0.1\\ 
    % +\textit{pELG} Top-5 No Mask &&&&&&&&&\\
    \midrule 
    \rowcolor{vvlightgray} 
    \textbf{Margin}, $\beta=1.2$ & 62.7 $\pm$ 0.6 & 79.4 $\pm$ 0.5 & 78.0 $\pm$ 0.3\\ 
    \hline
    +\textit{ELG} & 65.3 $\pm$ 0.5 & 83.2 $\pm$ 0.5 & 77.8 $\pm$ 0.1\\ 
    % +\textit{pELG} Top-1 & 64.9 $\pm$ 0.4 & 68.4 $\pm$ 0.4 & 33.0 $\pm$ 0.3 & 83.2 $\pm$ 0.4 & 68.7 $\pm$ 0.7 & 33.5 $\pm$ 0.3 & 78.1 $\pm$ 0.2  & 90.2 $\pm$ 0.3  & 46.3 $\pm$ 0.1 \\ 
    +\textit{PLG} Top-5 & 65.2 $\pm$ 0.5 & 83.4 $\pm$ 0.4 & 78.3 $\pm$ 0.2\\ 
    \midrule 
    \rowcolor{vvlightgray} 
    \textbf{Multisimilarity + S2SD} & 67.7 $\pm$ 0.3 & 86.5 $\pm$ 0.1 & 77.7 $\pm$ 0.2\\ 
    \hline
    +\textit{ELG} & 68.9 $\pm$ 0.4 & 88.2 $\pm$ 0.2 & 77.8 $\pm$ 0.1\\ 
    +\textit{PLG} Top-5 & 69.0 $\pm$ 0.4 & 88.4 $\pm$ 0.3 & 78.0 $\pm$ 0.1\\ 
    \bottomrule 

    \end{tabular}}
    \label{tab:relative_results}
    \vspace{-8pt}
 \end{table}




==> tables/sota_methods.tex <==
\begin{table*}[t]
    \caption{\textit{State-of-the-art.} \textbf{Bold}: best results per literature setup. The results showcase competitive and state-of-the-art performance with little hyperparameter tuning. 
    % We include NMI for comparability with previous methods, although it has been recently scrutinized regarding its expressivity and notable dependence on the utilized implementation \cite{musgrave2020metric}.
    While a separation into backbones and embedding dimensions provides a fairer comparison, we note some pipeline changes that improve performance independently and should be taken into account when comparing: \red{$^a$}: Better optimizer (RAdam \cite{radam} instead of Adam), \red{$^b$}: Larger input images, \red{$^c$}: Larger batchsizes on SOP, \red{$^d$}: Combination of pooling operations in backbone.}
    \vspace{-5pt}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l || c | c | c || c | c | c || c | c | c}
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks} $\rightarrow$} & \multicolumn{3}{c}{\textsc{CUB200} \cite{cub200-2011}} & \multicolumn{3}{c}{\textsc{CARS196} \cite{cars196}} & \multicolumn{3}{c}{\textsc{SOP} \cite{lifted}}\\
     \midrule
     \textsc{Methods} $\downarrow$ & R@1 & R@2 & NMI & R@1 & R@2 & NMI & R@1 & R@10 & NMI\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.9}}l}{\textbf{ResNet50, 128 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
     Margin \cite{margin}  & 63.6 & 74.4 & 69.0 & 79.6 & 86.5 & 69.1 & 72.7 & 86.2 & 90.7\\
    %  \rowcolor{vvlightgray}
     Div\&Conq \cite{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6 & 84.6 & 90.7 & 70.3 & 75.9 & 88.4 & 90.2\\
    %  \rowcolor{vvlightgray}
     MIC \cite{mic}                        & 66.1 & 76.8 & 69.7 & 82.6 & 89.1 & 68.4 & 77.2 & 89.4 & 90.0\\
    %  \rowcolor{vvlightgray}
     PADS \cite{roth2020pads}              & 67.3 & 78.0 & 69.9 & 83.5 & 89.7 & 68.8 & 76.5 & 89.0 & 89.9\\
    %  \rowcolor{vvlightgray}
     S2SD \cite{s2sd} & 68.9 $\pm$ 0.3 & 79.0 $\pm$ 0.3 & 72.1 $\pm$ 0.4 & 87.6 $\pm$ 0.2 & 92.7 $\pm$ 0.2 & 72.3 $\pm$ 0.2& 80.2 $\pm$ 0.2 & 91.5 $\pm$ 0.1 & 90.9 $\pm$ 0.1\\
     \hline
     Multisimilarity+\textit{PLG} & 67.8 $\pm$ 0.2 & 78.2 $\pm$ 0.2 & 70.1 $\pm$ 0.1 & 86.0 $\pm$ 0.3 & 91.4 $\pm$ 0.1 & 72.4 $\pm$ 0.2 & 77.9 $\pm$ 0.1 & 89.9 $\pm$ 0.2 & 90.2 $\pm$ 0.2\\     
     S2SD+\textit{PLG} & \textbf{71.1 $\pm$ 0.1} & \textbf{80.6 $\pm$ 0.2} & \textbf{73.0 $\pm$ 0.2} & \textbf{89.1 $\pm$ 0.2} & \textbf{93.8 $\pm$ 0.2} & \textbf{73.1 $\pm$ 0.3} & \textbf{80.6 $\pm$ 0.1} & \textbf{91.8 $\pm$ 0.2} & \textbf{90.9 $\pm$ 0.1}\\     
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.9}}l}{\textbf{ResNet50, 512 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
     EPSHN \cite{epshn}                     & 64.9 & 75.3 &  -   & 82.7 & 89.3 &  -  & 78.3 & 90.7 &  -    \\
    %  \rowcolor{vvlightgray}
     NormSoft \cite{zhai2018classification} & 61.3 & 73.9 &  -   & 84.2 & 90.4 &  -   & 78.2 & 90.6 &  -    \\
    %  \rowcolor{vvlightgray}
     DiVA \cite{milbich2020diva}            & 69.2 & 79.3 & 71.4 & 87.6 & 92.9 & 72.2 & 79.6 & 91.2 & 90.6 \\
    %  \rowcolor{vvlightgray}
     DCML-MDW \cite{Zheng_2021_CVPR_compositional} & 68.4 & 77.9 & 71.8 & 85.2 & 91.8 & 73.9 & 79.8 & 90.8 & 90.8 \\
    %  \rowcolor{vvlightgray}
     IB-DML \cite{seidenschwarz2021graphdml}\red{$^{a,b}$} & 70.3 & 80.3 & \textbf{74.0} & 88.1 & 93.3 & \textbf{74.8} & \textbf{81.4} & 91.3 & \textbf{92.6} \\     
    %  \rowcolor{vvlightgray}
    %  S2SD \cite{s2sd} & 70.1 $\pm$ 0.2 & 79.7 $\pm$ 0.2 & 71.6 $\pm$ 0.2 & 89.5 $\pm$ 0.2 & 93.9 $\pm$ 0.3 & 72.9 $\pm$ 0.3 & 81.0 $\pm$ 0.2 & 92.1 $\pm$ 0.2 & 91.1 $\pm$ 0.3\\
     \hline
     Multisimilarity+\textit{PLG} & 69.6 $\pm$  0.4 & 79.5 $\pm$ 0.2 & 70.7 $\pm$ 0.1 & 87.1 $\pm$ 0.2 & 92.3 $\pm$ 0.3 & 73.0 $\pm$ 0.2 & 79.0 $\pm$ 0.1 & 91.0 $\pm$ 0.1 & 90.0 $\pm$ 0.1\\     
     S2SD+\textit{PLG} & \textbf{71.4 $\pm$ 0.3} & \textbf{81.1 $\pm$ 0.2} & 73.5 $\pm$ 0.3 & \textbf{90.2 $\pm$ 0.3} & \textbf{94.4 $\pm$ 0.2} & 72.4 $\pm$ 0.3 & 81.3 $\pm$ 0.2 & \textbf{92.3 $\pm$ 0.2} & 91.1 $\pm$ 0.2\\     
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{10}{>{\columncolor[gray]{.9}}l}{\textbf{Inception-BN, 512 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$          & 66.3 & 76.7 & - & \\
    %  \rowcolor{vvlightgray}
    %  Softtriple \cite{softriple} & 65.4 & 76.4 & 69.3 & 84.5 & 90.7 & 70.1 & 78.3 & 90.3 & 92.0\\
    %  \rowcolor{vvlightgray}
     Group \cite{elezi2020grouploss} & 65.5 & 77.0 & 69.0 & 85.6 & 91.2 & \textbf{72.7} & 75.1 & 87.5 & 90.8   \\    
    %  \rowcolor{vvlightgray}          
     Multisimilarity\red{$^{c}$} \cite{multisimilarity} & 65.7 & 77.0 & - & 84.1 & 90.4 & -  & 78.2 & 90.5 & -   \\
    %  \rowcolor{vvlightgray}
     DR-MS \cite{dutta2020orthogonalunsupdml} & 66.1 & 77.0 & - & 85.0 & 90.5 & -  & - & - & -   \\
    %  \rowcolor{vvlightgray}     
    %  DiVA \cite{milbich2020diva} & 66.8 & 77.7 & 70.0 & 84.1 & 90.7 & 68.7  & 78.1 & 90.6 & 90.4   \\ 
    %  \rowcolor{vvlightgray}     
     ProxyGML \cite{Zhu2020graphdml} & 66.6 & 77.6 & 69.8 & 85.5 & 91.8 & 72.4  & 78.0 & 90.6 & 90.2   \\
    % %  \rowcolor{vvlightgray}     
     ProxyAnchor \cite{kim2020proxy}\red{$^{d}$} & 68.4 & 79.2 & - & 86.8 & 91.6 & -  & 79.1 & 90.8 & -   \\     
    %  \rowcolor{vvlightgray}
    %  S2SD \cite{s2sd} & 69.6 $\pm$ 0.3 & 79.6 $\pm$ 0.3 & 71.2 $\pm$ 0.1 & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2 & 79.1 $\pm$ 0.2 & 91.0 $\pm$ 0.3 & \textbf{90.4 $\pm$ 0.1}\\
     \hline
     Multisimilarity+\textit{PLG} & 69.2 $\pm$ 0.2 & 79.7 $\pm$ 0.1 & 70.6 $\pm$ 0.3 & 86.2 $\pm$ 0.2 & 91.5 $\pm$ 0.3 & 70.8 $\pm$ 0.3 & 78.6 $\pm$ 0.2 & 90.7 $\pm$ 0.1 & 90.0 $\pm$ 0.2 \\     
     S2SD+\textit{PLG} & \textbf{70.4 $\pm$ 0.2} & \textbf{80.5 $\pm$ 0.2} & \textbf{71.9 $\pm$ 0.3} & \textbf{88.1 $\pm$ 0.3} & \textbf{92.9 $\pm$ 0.1} & 71.4 $\pm$ 0.3 & \textbf{79.4 $\pm$ 0.1} & \textbf{91.2 $\pm$ 0.1} & \textbf{90.4 $\pm$ 0.2}\\            
     \bottomrule
\end{tabular}}

\vspace{-5pt}
\label{tab:sota}
\end{table*}




\begin{table*}[t]
    \caption{\textit{State-of-the-art.} \textbf{Bold}: best results per literature setup. The results showcase competitive and state-of-the-art performance with little hyperparameter tuning. 
    % We include NMI for comparability with previous methods, although it has been recently scrutinized regarding its expressivity and notable dependence on the utilized implementation \cite{musgrave2020metric}.
    While a separation into backbones and embedding dimensions provides a fairer comparison, we note some pipeline changes that improve performance independently and should be taken into account when comparing: \red{$^a$}: Better optimizer (RAdam \cite{radam} instead of Adam), \red{$^b$}: Larger input images, \red{$^c$}: Larger batchsizes on SOP, \red{$^d$}: Combination of pooling operations in backbone.}
    \vspace{-5pt}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l || c | c || c | c}
     \toprule
     \multicolumn{1}{l}{\textsc{Benchmarks} $\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200} \cite{cub200-2011}} & \multicolumn{2}{c}{\textsc{CARS196} \cite{cars196}}\\
     \midrule
     \textsc{Methods} $\downarrow$ & R@1 & R@2 & R@1 & R@2\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{ResNet50, 128 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
     Margin \cite{margin}  & 63.6 & 74.4 & 79.6 & 86.5\\
    %  \rowcolor{vvlightgray}
     Div\&Conq \cite{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 84.6 & 90.7\\
    %  \rowcolor{vvlightgray}
     MIC \cite{mic}                        & 66.1 & 76.8 & 82.6 & 89.1\\
    %  \rowcolor{vvlightgray}
     PADS \cite{roth2020pads}              & 67.3 & 78.0 & 83.5 & 89.7\\
    %  \rowcolor{vvlightgray}
     S2SD \cite{s2sd} & 68.9 $\pm$ 0.3 & 79.0 $\pm$ 0.3  & 87.6 $\pm$ 0.2 & 92.7 $\pm$ 0.2\\
     \hline
     Multisimilarity+\textit{PLG} & 67.8 $\pm$ 0.2 & 78.2 $\pm$ 0.2 & 86.0 $\pm$ 0.3 & 91.4 $\pm$ 0.1\\     
     S2SD+\textit{PLG} & \textbf{71.1 $\pm$ 0.1} & \textbf{80.6 $\pm$ 0.2} & \textbf{89.1 $\pm$ 0.2} & \textbf{93.8 $\pm$ 0.2}\\     
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{ResNet50, 512 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
     EPSHN \cite{epshn}                     & 64.9 & 75.3 & 82.7 & 89.3\\
    %  \rowcolor{vvlightgray}
     NormSoft \cite{zhai2018classification} & 61.3 & 73.9  & 84.2 & 90.4\\
    %  \rowcolor{vvlightgray}
     DiVA \cite{milbich2020diva}            & 69.2 & 79.3 & 87.6 & 92.9\\
    %  \rowcolor{vvlightgray}
     DCML-MDW \cite{Zheng_2021_CVPR_compositional} & 68.4 & 77.9 & 85.2 & 91.8\\
    %  \rowcolor{vvlightgray}
     IB-DML \cite{seidenschwarz2021graphdml}\red{$^{a,b}$} & 70.3 & 80.3 & 88.1 & 93.3\\     
    %  \rowcolor{vvlightgray}
    %  S2SD \cite{s2sd} & 70.1 $\pm$ 0.2 & 79.7 $\pm$ 0.2 & 71.6 $\pm$ 0.2 & 89.5 $\pm$ 0.2 & 93.9 $\pm$ 0.3 & 72.9 $\pm$ 0.3 & 81.0 $\pm$ 0.2 & 92.1 $\pm$ 0.2 & 91.1 $\pm$ 0.3\\
     \hline
     Multisimilarity+\textit{PLG} & 69.6 $\pm$  0.4 & 79.5 $\pm$ 0.2 & 87.1 $\pm$ 0.2 & 92.3 $\pm$ 0.3\\     
     S2SD+\textit{PLG} & \textbf{71.4 $\pm$ 0.3} & \textbf{81.1 $\pm$ 0.2}& \textbf{90.2 $\pm$ 0.3} & \textbf{94.4 $\pm$ 0.2}\\     
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{5}{>{\columncolor[gray]{.9}}l}{\textbf{Inception-BN, 512 dim.}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$          & 66.3 & 76.7 & - & \\
    %  \rowcolor{vvlightgray}
    %  Softtriple \cite{softriple} & 65.4 & 76.4 & 69.3 & 84.5 & 90.7 & 70.1 & 78.3 & 90.3 & 92.0\\
    %  \rowcolor{vvlightgray}
     Group \cite{elezi2020grouploss} & 65.5 & 77.0 & 85.6 & 91.2\\    
    %  \rowcolor{vvlightgray}          
     Multisimilarity\red{$^{c}$} \cite{multisimilarity} & 65.7 & 77.0& 84.1 & 90.4\\
    %  \rowcolor{vvlightgray}
     DR-MS \cite{dutta2020orthogonalunsupdml} & 66.1 & 77.0 & 85.0 & 90.5\\
    %  \rowcolor{vvlightgray}     
    %  DiVA \cite{milbich2020diva} & 66.8 & 77.7 & 70.0 & 84.1 & 90.7 & 68.7  & 78.1 & 90.6 & 90.4   \\ 
    %  \rowcolor{vvlightgray}     
     ProxyGML \cite{Zhu2020graphdml} & 66.6 & 77.6 & 85.5 & 91.8\\
    % %  \rowcolor{vvlightgray}     
     ProxyAnchor \cite{kim2020proxy}\red{$^{d}$} & 68.4 & 79.2 & 86.8 & 91.6\\     
    %  \rowcolor{vvlightgray}
    %  S2SD \cite{s2sd} & 69.6 $\pm$ 0.3 & 79.6 $\pm$ 0.3 & 71.2 $\pm$ 0.1 & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2 & 79.1 $\pm$ 0.2 & 91.0 $\pm$ 0.3 & \textbf{90.4 $\pm$ 0.1}\\
     \hline
     Multisimilarity+\textit{PLG} & 69.2 $\pm$ 0.2 & 79.7 $\pm$ 0.1 & 86.2 $\pm$ 0.2 & 91.5 $\pm$ 0.3\\     
     S2SD+\textit{PLG} & \textbf{70.4 $\pm$ 0.2} & \textbf{80.5 $\pm$ 0.2} & \textbf{88.1 $\pm$ 0.3} & \textbf{92.9 $\pm$ 0.1}\\            
     \bottomrule
\end{tabular}}

\vspace{-5pt}
\label{tab:sota}
\end{table*}
